This PIN Can Be Easily Guessed: Analyzing the Security of Smartphone Unlock PINs

In this paper, we provide the first comprehensive study of user-chosen 4- and 6-digit PINs (n=1220) collected on smartphones with participants being explicitly primed for device unlocking. We find that against a throttled attacker (with 10, 30, or 100 guesses, matching the smartphone unlock setting), using 6-digit PINs instead of 4-digit PINs provides little to no increase in security, and surprisingly may even decrease security. We also study the effects of blocklists, where a set of "easy to guess" PINs is disallowed during selection. Two such blocklists are in use today by iOS, for 4-digits (274 PINs) as well as 6-digits (2910 PINs). We extracted both blocklists compared them with four other blocklists, including a small 4-digit (27 PINs), a large 4-digit (2740 PINs), and two placebo blocklists for 4- and 6-digit PINs that always excluded the first-choice PIN. We find that relatively small blocklists in use today by iOS offer little or no benefit against a throttled guessing attack. Security gains are only observed when the blocklists are much larger, which in turn comes at the cost of increased user frustration. Our analysis suggests that a blocklist at about 10% of the PIN space may provide the best balance between usability and security.

==> fig/plots/warning/app.tex <==
\definecolor{exp_strongly_agree}{HTML}{3598DB} % blue
\definecolor{exp_agree}{HTML}{9ACCED}
\definecolor{exp_neutral}{HTML}{A0A0A0}
\definecolor{exp_disagree}{HTML}{F9F5C3}
\definecolor{exp_strongly_disagree}{HTML}{EBDF42} % yellow

\definecolor{img_strongly_agree}{HTML}{549C77} % green
\definecolor{img_agree}{HTML}{ABD4B4}
\definecolor{img_neutral}{HTML}{A0A0A0}
\definecolor{img_disagree}{HTML}{E5B8FF}
\definecolor{img_strongly_disagree}{HTML}{950095} % purple

\begin{figure*}[h]
\small
\centering
\renewcommand*{\arraystretch}{0.5}
    \centering
    \setlength{\tabcolsep}{0pt}

    \begin{tabular}{r c c}
        \toprule
        \textbf{Treatment} & \textbf{Is Appropriate to Display Warning} & \textbf{Would Be Appropriate to Display Warning}\\
        \midrule

\raisebox{0.3em}{\fourControlAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(41.1255411255,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(41.9913419913,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(12.5541125541,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(2.5974025974,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(1.7316017316,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourPlaceboAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(36.8852459016,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(31.9672131148,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(23.7704918033,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(5.73770491803,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(1.6393442623,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourIosNoAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(52.380952381,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(14.2857142857,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(19.0476190476,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(9.52380952381,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(4.7619047619,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(32.380952381,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(47.619047619,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(12.380952381,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(4.7619047619,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(2.85714285714,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourIosWithAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(50.0,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(32.1428571429,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(14.2857142857,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(3.57142857143,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(35.4166666667,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(42.7083333333,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(9.375,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(8.33333333333,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(4.16666666667,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourDataSmallAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(80.0,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(20.0,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(36.2068965517,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(50.0,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(6.89655172414,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(5.1724137931,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(1.72413793103,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourDataLargeAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(37.5,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(29.5454545455,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(20.4545454545,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(7.95454545455,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(4.54545454545,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(28.2051282051,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(48.7179487179,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(12.8205128205,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(5.12820512821,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(5.12820512821,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\sixControlAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(40.157480315,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(44.8818897638,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(8.66141732283,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(3.93700787402,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(2.36220472441,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\sixPlaceboAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(39.3162393162,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(42.735042735,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(11.1111111111,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(6.83760683761,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{3.5em}{\sixIosWithAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(73.3333333333,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(13.3333333333,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(6.66666666667,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(6.66666666667,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\addlegendentry{Strongly\\Agree};
\addlegendentry{Agree};
\addlegendentry{Neutral};
\addlegendentry{Disagree};
\addlegendentry{Strongly\\Disagree};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(33.6363636364,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(50.0,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(12.7272727273,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(2.72727272727,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(0.909090909091,1)};
\addlegendentry{Strongly\\Agree};
\addlegendentry{Agree};
\addlegendentry{Neutral};
\addlegendentry{Disagree};
\addlegendentry{Strongly\\Disagree};
\end{axis}
\end{tikzpicture}} \\

    \bottomrule
    \end{tabular}
    \caption{Responses of participants for the question: ``\emph{It is appropriate for smartphones to display warning messages about PIN security.}'' We split the participants by those who hit and those who have \underline{not} hit a blacklist. One can observe that the majority of participants consider it to be okay if a warning about weak PIN choice shows up on a smartphone.}\label{fig:warning-appropriate}
\end{figure*}


==> fig/plots/warning/cause.tex <==
\definecolor{exp_strongly_agree}{HTML}{3598DB} % blue
\definecolor{exp_agree}{HTML}{9ACCED}
\definecolor{exp_neutral}{HTML}{A0A0A0}
\definecolor{exp_disagree}{HTML}{F9F5C3}
\definecolor{exp_strongly_disagree}{HTML}{EBDF42} % yellow

\definecolor{img_strongly_agree}{HTML}{549C77} % green
\definecolor{img_agree}{HTML}{ABD4B4}
\definecolor{img_neutral}{HTML}{A0A0A0}
\definecolor{img_disagree}{HTML}{E5B8FF}
\definecolor{img_strongly_disagree}{HTML}{950095} % purple

\begin{figure*}[h]
\centering
\small
\renewcommand*{\arraystretch}{0.5}
    \centering
    \setlength{\tabcolsep}{0pt}

    \begin{tabular}{r c c}
        \toprule
        \textbf{Treatment} & \textbf{Creation Strategy Caused Warning} & \textbf{Creation Strategy Would Cause Warning}\\
        \midrule

\raisebox{0.3em}{\fourControlAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(12.987012987,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(27.7056277056,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(19.9134199134,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(28.5714285714,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(10.8225108225,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourPlaceboAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(30.3278688525,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(31.1475409836,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(18.0327868852,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(12.2950819672,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(8.19672131148,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourIosNoAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(28.5714285714,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(57.1428571429,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(4.7619047619,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(9.52380952381,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(1.90476190476,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(20.0,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(22.8571428571,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(39.0476190476,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(16.1904761905,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourIosWithAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(71.4285714286,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(14.2857142857,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(10.7142857143,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(3.57142857143,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(5.20833333333,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(21.875,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(29.1666666667,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(27.0833333333,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(16.6666666667,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourDataSmallAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(60.0,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(40.0,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(10.3448275862,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(24.1379310345,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(16.3793103448,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(35.3448275862,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(13.7931034483,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\fourDataLargeAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(48.8636363636,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(34.0909090909,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(3.40909090909,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(5.68181818182,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(7.95454545455,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(10.2564102564,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(17.9487179487,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(15.3846153846,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(41.0256410256,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(15.3846153846,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\sixControlAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(11.0236220472,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(25.9842519685,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(18.1102362205,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(29.9212598425,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(14.9606299213,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{0.3em}{\sixPlaceboAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(36.7521367521,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(33.3333333333,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(10.2564102564,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(11.1111111111,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(8.54700854701,1)};
\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5},xticklabel style={opacity=0,yshift=10pt}]
\addplot[draw=black,fill=white] coordinates {(100,1)};
\end{axis}
\end{tikzpicture}} \\

\raisebox{3.5em}{\sixIosWithAbbr} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5}]
\addplot[fill=exp_strongly_agree, xbar legend, mark=none] coordinates {(60.0,1)};
\addplot[fill=exp_agree, xbar legend, mark=none] coordinates {(40.0,1)};
\addplot[fill=exp_neutral, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\addplot[fill=exp_strongly_disagree, xbar legend, mark=none] coordinates {(0.0,1)};
\addlegendentry{Strongly\\Agree};
\addlegendentry{Agree};
\addlegendentry{Neutral};
\addlegendentry{Disagree};
\addlegendentry{Strongly\\Disagree};

\end{axis}
\end{tikzpicture}} & \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[xbar stacked,bar width=0.29cm,ytick=\empty,y post scale=0.05,xmin=0,xmax=100,legend style={at={(0,-3)},
legend style={cells={align=left, anchor=center, fill}, nodes={inner sep=0.4ex,below=-2ex}},
column sep=0cm, draw=none, anchor=west, legend columns=5}]
\addplot[fill=img_strongly_agree, xbar legend, mark=none] coordinates {(8.18181818182,1)};
\addplot[fill=img_agree, xbar legend, mark=none] coordinates {(23.6363636364,1)};
\addplot[fill=img_neutral, xbar legend, mark=none] coordinates {(25.4545454545,1)};
\addplot[fill=img_disagree, xbar legend, mark=none] coordinates {(31.8181818182,1)};
\addplot[fill=img_strongly_disagree, xbar legend, mark=none] coordinates {(10.9090909091,1)};
\addlegendentry{Strongly\\Agree};
\addlegendentry{Agree};
\addlegendentry{Neutral};
\addlegendentry{Disagree};
\addlegendentry{Strongly\\Disagree};
\end{axis}
\end{tikzpicture}} \\

    \bottomrule
    \end{tabular}
\caption{Most participants were asked to rate their agreement, using a 5-point Likert scale to the statement: ``\emph{My initial PIN creation strategy caused the display of this warning.}'' For the other participants who have \underline{not} hit a blacklist: ``\emph{My PIN creation strategy would cause this warning message to appear.}'' One can observe that participants in general have difficulties imagining that their PIN choice could be considered insecure.}\label{fig:warning-cause}
\end{figure*} 
